A Survey of Knowledge-Intensive NLP with Pre-Trained Language Models

With the increasing of model capacity brought by pre-trained language models, there emerges boosting needs for more knowledgeable natural language processing (NLP) models with advanced functionalities including providing and making flexible use of encyclopedic and commonsense knowledge. The mere pre-trained language models, however, lack the capacity of handling such knowledge-intensive NLP tasks alone. To address this challenge, large numbers of pre-trained language models augmented with external knowledge sources are proposed and in rapid development. In this paper, we aim to summarize the current progress of pre-trained language model-based knowledge-enhanced models (PLMKEs) by dissecting their three vital elements: knowledge sources, knowledge-intensive NLP tasks, and knowledge fusion methods. Finally, we present the challenges of PLMKEs based on the discussion regarding the three elements and attempt to provide NLP practitioners with potential directions for further research.

==> sections/backup.tex <==
\begin{table}[!ht]
\centering
\scriptsize
\scalebox{0.86}{
\begin{tabular}{ccc}
\toprule
\textbf{Dataset} & \textbf{Data Source}   & \textbf{Needed Knowledge} \\
\midrule
\begin{tabular}[c]{@{}c@{}}\textsc{FEVER}\\ \cite{thorne-etal-2018-fever}\end{tabular}       & Wikipedia & \multirow{3}{*}[-1.7em]{\makecell[c]{general factual knowledge \\ (e.g., Wikipedia, social media, etc.)}} \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{BoolQ} \\ \cite{clark-etal-2019-boolq}\end{tabular}       & Wikipedia &  \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{UKPSnopes} \\ \cite{hanselowski-etal-2019-richly}\end{tabular}       & Snopes website &  \\
\cmidrule(lr{1em}){1-3}
\begin{tabular}[c]{@{}c@{}}\textsc{Emergent} \\ \cite{ferreira-vlachos-2016-emergent}\end{tabular}       & \makecell[c]{Snopes website \& \\ Twitter} &  news \& tech stories \\
\cmidrule(lr{1em}){1-3}
\begin{tabular}[c]{@{}c@{}}\textsc{PolitiFact14} \\ \cite{vlachos-riedel-2014-fact}\end{tabular}       & \makecell[c]{PolitiFact \& \\ Channel 4 websites} & \makecell[c]{news \& government reports, etc.} \\
\cmidrule(lr{1em}){1-3}
\begin{tabular}[c]{@{}c@{}}\textsc{COVID-Fact} \\ \cite{saakyan-etal-2021-covid}\end{tabular}       & \makecell[c]{Reddit \& Google search \\ results about COVID} & \makecell[c]{COVID-related articles \\ and discussions} \\
\cmidrule(lr{1em}){1-3}
\begin{tabular}[c]{@{}c@{}}\textsc{SciFact} \\ \cite{wadden-etal-2020-fact}\end{tabular}       & \makecell[c]{Scientific articles} & \makecell[c]{scientific knowledge about \\ biology, medicine, etc.} \\
\bottomrule
\end{tabular}
}
\caption{Detailed information about representative fact verification datasets.}
\end{table}

\begin{table}[!ht]
\centering
\scriptsize
\begin{tabular}{ccc}
\toprule
\textbf{Dataset} & \textbf{Data Source}   & \textbf{Needed Knowledge} \\
\midrule
\begin{tabular}[c]{@{}c@{}}\textsc{ACE2004} \\ \cite{nist2004}\end{tabular}       & \makecell[c]{Wikipedia} &  \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{AIDA CoNLL-YAGO} \\ \cite{hoffart-etal-2011-robust}\end{tabular}       & DBPedia \& YAGO & \multirow{4}{*}[0em]{\makecell[c]{general factual knowledge \\ (e.g., Wikipedia, DBPedia, etc.)}} \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{WnWi}\\ \cite{DBLP:conf/cikm/GuoB14}\end{tabular}       & Wikipedia &  \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{WnCw} \\ \cite{DBLP:conf/cikm/GuoB14}\end{tabular}       & Clueweb &  \\
\cmidrule(lr{1em}){1-3}
\begin{tabular}[c]{@{}c@{}}\textsc{WikiMed} \\ \cite{medtype2020}\end{tabular}       & \makecell[c]{Wikipedia \& \\ UMLS} & \makecell[c]{biomedical knowledge} \\
\bottomrule
\end{tabular}
\caption{Detailed information about representative entity disambiguation datasets.}
\end{table}

\begin{table}[!ht]
\centering
\scriptsize
\begin{threeparttable}
\begin{tabular}{cccc}
\toprule
\textbf{Dataset} & \textbf{Data Source}   & \textbf{Needed Knowledge} \\
\midrule
\textsc{Google-RE}\tnote{1}       & \makecell[c]{Wikipedia} &  \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{T-REx} \\ \cite{elsahar-etal-2018-rex}\end{tabular}       & Wikipedia \& DBPedia & \multirow{3}{*}[0.5em]{\makecell[c]{general factual knowledge \\ (e.g., Wikipedia, DBPedia, etc.)}} \\
\cmidrule(lr{1em}){1-2}
\begin{tabular}[c]{@{}c@{}}\textsc{Zero-shot RE}\\ \cite{levy-etal-2017-zero}\end{tabular}       & Wikipedia &  \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\scriptsize
\item[1] \url{https://code.google.com/archive/p/relation-extraction-corpus/}
\end{tablenotes}
\end{threeparttable}
\caption{Detailed information about representative knowledge triplet slot filling datasets.}
\end{table}

\subsection{Commonsense Knowledge-aware Tasks}
